Narrative Action Evaluation with Prompt-Guided Multimodal Interaction

In this paper, we investigate a new problem called narrative action evaluation (NAE). NAE aims to generate professional commentary that evaluates the execution of an action. Unlike traditional tasks such as score-based action quality assessment and video captioning involving superficial sentences, NAE focuses on creating detailed narratives in natural language. These narratives provide intricate descriptions of actions along with objective evaluations. NAE is a more challenging task because it requires both narrative flexibility and evaluation rigor. One existing possible solution is to use multi-task learning, where narrative language and evaluative information are predicted separately. However, this approach results in reduced performance for individual tasks because of variations between tasks and differences in modality between language information and evaluation information. To address this, we propose a prompt-guided multimodal interaction framework. This framework utilizes a pair of transformers to facilitate the interaction between different modalities of information. It also uses prompts to transform the score regression task into a video-text matching task, thus enabling task interactivity. To support further research in this field, we re-annotate the MTL-AQA and FineGym datasets with high-quality and comprehensive action narration. Additionally, we establish benchmarks for NAE. Extensive experiment results prove that our method outperforms separate learning methods and naive multi-task learning methods. Data and code are released at https://github.com/shiyi-zh0408/NAE_CVPR2024.

==> figures/overview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/teasor_2.png}
    % \vspace{-5pt}
    \caption{A comparison of narrative action evaluation (NAE) with action quality assessment (AQA) and video captioning. NAE includes much more evaluation information such as \textcolor[RGB]{192,0,0}{\textbf{\underline{\textit{scores}}}}, \textcolor[RGB]{197,90,17}{\textbf{\underline{\textit{qualitative evaluations}}}}, \textcolor[RGB]{47,85,151}{\textbf{\underline{\textit{action descriptions}}}}, and so on. While generating descriptive language, NAE needs to take the accuracy of evaluation information (such as scores) into account. However, such assessment information is often rigorous and granular. Despite their importance, their proportion in sentences is small, so NAE may be difficult to tackle through traditional video captioning methods.}
    \label{fig:overview}
    % \vspace{-10pt}
\end{figure*}

==> figures/rebuttal_attend_fig_tab.tex <==
% \begin{figure}[h]
%     \vspace{-10pt}
%     \begin{minipage}[b]{0.1\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{imgs/rebuttal_mask_3.pdf}
%     % \caption{Fig}
%     \end{minipage}
%     \raisebox{23pt}{
%         \begin{minipage}[b]{0.2\textwidth}
%         \centering
%             % \scriptsize
%             % \renewcommand\arraystretch{1.4}
%             % \begin{center}
%             \setlength{\tabcolsep}{3pt}
%             \vspace{-80pt}
%              \setlength{\tabcolsep}{3.9mm}{
%              \scalebox{0.83}{
%             \begin{tabular}{l|ccc}
%             \toprule
%             Token&   Word&Temp.&Video\\ 
%             \midrule
%             Word&   \ding{51}(causal)&\ding{51}&\ding{51}\\
%             Temp.&   \ding{55}&\ding{51}&\ding{51}\\
%             Video&   \ding{55}&\ding{55}&\ding{51}(sparse)\\
%             \bottomrule
%             \end{tabular}}}\label{tab:rebuttal_attend}
%         \end{minipage}
%     }
%     \vspace{-10pt}
% \end{figure}

\setlength{\intextsep}{2pt} % 设置图片与文本的垂直距离
\setlength{\columnsep}{4pt} % 设置图片与文本之间的水平距离

\begin{wrapfigure}{r}[0em]{0.275\textwidth}
    \vspace{-5pt}
    \begin{minipage}[b]{0.073\textwidth}
    \centering
    \includegraphics[width=\textwidth]{imgs/rebuttal_mask_3.pdf}
    % \caption{Fig}
    \end{minipage}
    \raisebox{16.5pt}{
        \hspace{-10pt}
        \begin{minipage}[b]{0.2\textwidth}
        \centering
            \vspace{-3pt}
            \fontsize{7}{12}\selectfont \renewcommand{\arraystretch}{0.67}
             \setlength{\tabcolsep}{0.8mm}{
             \scalebox{0.8}{
            \begin{tabular}{l|ccc}
            \toprule
            Token&   Word&Temp.&Video\\ 
            \midrule
            Word&   \ding{51}(causal)&\ding{51}&\ding{51}\\
            Temp.&   \ding{55}&\ding{51}&\ding{51}\\
            Video&   \ding{55}&\ding{55}&\ding{51}(sparse)\\
            \bottomrule
            \end{tabular}}}\label{tab:rebuttal_attend}
        \end{minipage}
    }
    \vspace{-10pt}
\end{wrapfigure}


==> figures/rebuttal_case_fig1.tex <==
\begin{figure}[h]
    \vspace{0pt}
    \centering
    \setlength{\abovecaptionskip}{0.cm}
    \includegraphics[width=1\linewidth]{imgs/rebuttal_case_fig1_2.pdf}
    \label{fig:re_case1}
    \vspace{-25pt}
\end{figure}

==> figures/rebuttal_case_fig2.tex <==
\begin{figure}[h]
    \vspace{2pt}
    \centering
    \setlength{\abovecaptionskip}{0.cm}
    \includegraphics[width=1\linewidth]{imgs/rebuttal_case_fig2_2.pdf}
    \label{fig:re_case2}
    \vspace{-32pt}
\end{figure}

==> figures/rebuttal_mask.tex <==
\setlength{\intextsep}{2pt} % 设置图片与文本的垂直距离
\setlength{\columnsep}{4pt} % 设置图片与文本之间的水平距离

\begin{wrapfigure}{r}[0em]{0.2\textwidth}%靠文字内容的右侧
\centering
\vspace{-20pt}
\includegraphics[width=0.2\textwidth]{imgs/rebuttal_mask_1.pdf}
\label{fig:rebuttal_mask}
\vspace{-30pt}
\end{wrapfigure}


==> figures/sup_case1.tex <==
\begin{figure*}[b]
    \centering
    \includegraphics[width=\linewidth]{imgs/sup_case1.pdf}
    % \vspace{-5pt}
    \caption{\textbf{Qualitative Results (a).} Our model can generate detailed narrations to describe and evaluate the actions comprehensively. Notably, the model can analyze the quality of actions by pointing out the details of the execution.}
    \label{fig:newcase1}
    % \vspace{-0.5cm}
\end{figure*}

==> figures/sup_case2.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{imgs/sup_case2.pdf}
    % \vspace{-5pt}
    \caption{\textbf{Qualitative Results (b).} Our model can generate detailed narrations to describe and evaluate the actions comprehensively. Notably, the model can analyze the quality of actions by pointing out the details of the execution.}
    \label{fig:newcase2}
    % \vspace{-0.5cm}
\end{figure*}

==> figures/sup_case3.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/sup_case3.pdf}
    % \vspace{-5pt}
    \caption{\textbf{Qualitative Results (c).} Our model can generate detailed narrations to describe and evaluate the actions comprehensively. Notably, the model can analyze the quality of actions by pointing out the details of the execution.}
    \label{fig:newcase3}
    % \vspace{-0.5cm}
\end{figure*}

==> figures/sup_dataset1.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/sup_dataset1.pdf}
    % \vspace{-5pt}
    \caption{\textbf{Qualitative Results.} Our model can generate detailed narrations to describe and evaluate the actions comprehensively. Notably, the model can analyze the quality of actions by pointing out the details of the execution.}
    \label{fig:dataset1}
    % \vspace{-0.5cm}
\end{figure*}

==> figures/sup_dataset2.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/sup_dataset2.pdf}
    % \vspace{-5pt}
    \caption{\textbf{Prompt (b).} The five versions of prompts we use to guide ChatGPT in generating different forms of text. And comparisons of the text before and after re-annotation.}
    \label{fig:dataset2}
    % \vspace{-0.5cm}
\end{figure}

==> tables/ablation_all.tex <==
\begin{minipage}[t]{\textwidth}
\begin{minipage}[t]{0.33\textwidth}
\makeatletter\def\@captype{table}
\begin{center} 
% \captionsetup{font=small}
\caption{Impact of different framework components}
\vspace{5pt}
\small \renewcommand{\arraystretch}{0.67}%修改表格行间距和字号(紧凑版本)
\setlength{\tabcolsep}{1mm}{ % 修改表格宽度
% \setlength{\tabcolsep}{1.4mm}{ % 修改表格宽度(紧凑版本)
\begin{tabular}{cccc}
\toprule
w/o Module & B4 & M & C \\ 
\midrule
Le.Pr  & 41.81 & 27.70 & 18.47 \\
C-Attn1 & 41.46 & 27.37 & 19.08 \\
C-Attn2 & 41.73 & 27.69 & 19.68 \\
\midrule
\textbf{full model}& \textbf{42.23} & \textbf{28.22} & \textbf{20.54} \\
% \ding{51} & \ding{51} & \ding{51} & \ding{51}  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}}
% \vspace{4pt}
\label{tab:frameworkablation}
\end{center}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\makeatletter\def\@captype{table}
\begin{center}
% \captionsetup{font=small}
\caption{Impact of different loss functions}
\vspace{7pt}
\small \renewcommand{\arraystretch}{0.67}%修改表格行间距和字号(紧凑版本)
\setlength{\tabcolsep}{1.5mm}{ % 修改表格宽度
% \setlength{\tabcolsep}{1.4mm}{ % 修改表格宽度(紧凑版本)
\begin{tabular}{cccc}
\toprule
w/o Loss & B4 & M & C \\ 
\midrule
CE & 41.56 & 27.35 & 19.22 \\
MSE & 41.62 & 27.32 & 18.96 \\
CE+MSE & 41.38 & 27.44 & 18.74 \\
\midrule
\textbf{full model}& \textbf{42.23} & \textbf{28.22} & \textbf{20.54} \\
\bottomrule
\end{tabular}}
\label{tab:lossablation}
\end{center}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\makeatletter\def\@captype{table}
% \captionsetup{font=small}
\caption{Impact of different template}
\small \renewcommand{\arraystretch}{0.67}%修改表格行间距和字号(紧凑版本)
\begin{center} 
% \setlength{\tabcolsep}{0.5mm}{ % 修改表格宽度
\setlength{\tabcolsep}{1.5mm}{ % 修改表格宽度(紧凑版本)
\begin{tabular}{cccccc}
\toprule
Template &  B4 & M & C \\ 
\midrule
Sco. & 37.57 & 26.47 & 15.22 \\
Act. & 40.48 & 27.86 & 19.64 \\
  & 40.17 & 26.38 & 16.21 \\
\midrule
\textbf{Sco.+Act.} & \textbf{42.23} & \textbf{28.22} & \textbf{20.54} \\
\bottomrule
\end{tabular}}
\label{tab:templateablation}
\end{center}
\end{minipage}
\end{minipage}

% \usepackage{floatrow}
% \floatsetup[table]{capposition=top}
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]

% \begin{table*}
% \begin{floatrow}
% % \begin{center} 
% \capbtabbox{
% \small \renewcommand{\arraystretch}{0.67}%修改表格行间距和字号(紧凑版本)
% \setlength{\tabcolsep}{0.6mm}{ % 修改表格宽度
% % \setlength{\tabcolsep}{1.4mm}{ % 修改表格宽度(紧凑版本)
% \begin{tabular}{cccc}
% \toprule
% w/o Module & B4 & M & C \\ 
% \midrule
% Le.Pr  & 41.81 & 27.70 & 18.47 \\
% C-Attn & 41.46 & 27.37 & 19.08 \\
% Sco.Pred. & 41.38 & 27.44 & 18.74 \\
% \midrule
% & 42.35 & 27.78 & 20.25 \\
% % \ding{51} & \ding{51} & \ding{51} & \ding{51}  &  &  &  &  &  &  &  \\
% \bottomrule
% \end{tabular}}
% \caption{Impact of different framework components}
% \label{tab:frameworkablation}
% }
% % \end{center}
% {
%  \caption{Table 1. }
%  \label{Tab1}
% }

% \capbtabbox{
% \small \renewcommand{\arraystretch}{0.67}%修改表格行间距和字号(紧凑版本)
% \setlength{\tabcolsep}{0.6mm}{ % 修改表格宽度
% % \setlength{\tabcolsep}{1.4mm}{ % 修改表格宽度(紧凑版本)
% \begin{tabular}{cccc}
% \toprule
% w/o Loss & B4 & M & C \\ 
% \midrule
% ce & 41.56 & 27.35 & 19.22 \\
% mse & 41.62 & 27.32 & 18.96 \\
% ce+mse & 41.38 & 27.44 & 18.74 \\
% \midrule
% & 42.35 & 27.78 & 20.25 \\
% \bottomrule
% \end{tabular}}
% \caption{Impact of different loss functions}
% \label{tab:lossablation}
% }{
%  \caption{Table 2.}
%  \label{Tab2}
%  \small
% }

% \capbtabbox{
% \small \renewcommand{\arraystretch}{0.67}%修改表格行间距和字号(紧凑版本)
% % \begin{center} 
% % \setlength{\tabcolsep}{0.5mm}{ % 修改表格宽度
% \setlength{\tabcolsep}{0.6mm}{ % 修改表格宽度(紧凑版本)
% \begin{tabular}{cccccc}
% \toprule
% Template &  B4 & M & C \\ 
% \midrule
% Sco. &  &  &  \\
% Act. &  &  &  \\
%   & 40.17 & 26.38 & 16.21 \\
% \midrule
% Sco.+Act. & 41.39 & 27.92 & 20.48 \\
% \bottomrule
% \end{tabular}}
% \caption{Impact of different template}
% \label{tab:templateablation}
% }
% % \end{center}
% {
%  \caption{Table 1. }
%  \label{Tab1}
% }

% \end{floatrow}
% \end{table*}
